Improving Hierarchical Adversarial Robustness of Deep Neural Networks

Do all adversarial examples have the same consequences? An autonomous driving system misclassifying a pedestrian as a car may induce a far more dangerous -- and even potentially lethal -- behavior than, for instance, a car as a bus. In order to better tackle this important problematic, we introduce the concept of hierarchical adversarial robustness. Given a dataset whose classes can be grouped into coarse-level labels, we define hierarchical adversarial examples as the ones leading to a misclassification at the coarse level. To improve the resistance of neural networks to hierarchical attacks, we introduce a hierarchical adversarially robust (HAR) network design that decomposes a single classification task into one coarse and multiple fine classification tasks, before being specifically trained by adversarial defense techniques. As an alternative to an end-to-end learning approach, we show that HAR significantly improves the robustness of the network against $\ell_2$ and $\ell_{\infty}$ bounded hierarchical attacks on the CIFAR-10 and CIFAR-100 dataset.

==> _related.tex <==
Our work introduces a novel architectural approach to improve hierarchical adversarial robustness of neural networks.
% 
It is inspired by the recent advances in adversarial learning research and early work in exploiting class hierarchy of dataset for different downstream tasks.

% \subsection{Adversarial Defence Methods}
A plethora of defence mechanisms have been proposed for the adversarial setting.
% 
Adversarial training~\citep{szegedy2013intriguing} is one of the standard approaches for improving the robustness of deep neural networks against adversarial examples.
%
It is a data augmentation method that replaces unperturbed training data with adversarial examples and updates the network with the replaced data points.
%
Intuitively, this procedure encourages the DNN not to make the same mistakes against an adversary.
%
By adding sufficiently enough adversarial examples, the network gradually becomes robust to the attack it was trained on.
% 
Existing adversarial training methods ~\citep{szegedy2013intriguing, goodfellow2014explaining, kurakin2016adversarial, madry2017towards, wong2020fast} differ in the adversaries used in the training.
% 
Another related line of adversarial defence methods focuses on regularizing the loss function instead of data augmentation.
% 
TRADES~\citep{zhang2019theoretically} introduces a regularization term that penalizes the difference between the output of the model on a training data and its corresponding adversarial example. 
% 
The regularized loss consists of a standard cross-entropy loss on the unperturbed data and a KL-divergence term measuring the difference between the distribution of clean training data and adversarially perturbed training data.
% 
% Although newer defence methods exist, adversarial training and TRADES remain popular as the benchmarks.

% \subsection{Image Classification with Class Hierarchy}
In image classification domain, there is a sizable body of work exploiting class hierarchy of the dataset~\citep{tousch2012semantic}. 
% 
For classification with a large number of classes, it is a common technique to divide the end-to-end learning task into multiple classifications based on the semantic hierarchy of the labels~\citep{marszalek2008constructing, liu2013probabilistic, deng2012hedging}.
% 
They are motivated by the intuition that some coarse labels are more difficult to distinguish than others, and specific category of classes requires more dedicated classifiers.
% 
A popular hierarchy structure is to divide the fine labels into a label tree with root nodes and leaf nodes. 
% 
\cite{deng2011fast} propose an efficient technique to simultaneously determine the structure of the tree as well as learning the classifier for each node in the tree.
%
Instead of learning the optimal tree structure, it is also common to use the predefined hierarchy of the dataset~\cite{deng2012hedging}.
% 

% Often, such approaches allow training multiple smaller networks in parallel. However, the decreased training time comes at the expense of losing accuracy.
% 




==> table_dumpster.tex <==
\begin{table*}[h]
\begin{footnotesize}
\caption{Performance on CIFAR-10 and CIFAR100-subset against $\ell_{\infty}$ bounded transferred attacks ($\eps = 8/255$). }
\label{table:parent_attack}
%\vskip 0.15in
\begin{center}
\setlength{\tabcolsep}{15pt} % Default value: 6pt (space between columns)
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{tabular}{llllll}
                         & \multicolumn{2}{c}{Method} 					& Standard 	  & ADV 		   & TRADES 		\\ \Xhline{2\arrayrulewidth}
\multirow{6}{*}{\rotatebox{90}{CIFAR-10}} & \multirow{3}{*}{Vanilla}         & Standard  & $32.99\%$   & $81.25\%$      & $89.72\%$ 	 \\
                         &                                 					& ADV       & $96.88\%$   & $78.16\%$     & $89.34\%$  	 \\
                         &                                 					& TRADES    & $95.03\%$   & $73.57\%$     & $88.05\%$   	\\ \cline{2-6}
                         & \multirow{3}{*}{HR}   							& Standard  & $49.21\%$   & $82.96\%$      & $92.63\%$ 	 \\
                         &                                 					& ADV       & $95.36\%$   & $76.11\%$     & $90.49\%$  	 \\
                         &                                 					& TRADES    & $94.37\%$   & $74.71\%$     & $90.89\%$   	\\  \hline \hline

\multirow{6}{*}{\rotatebox{90}{CIFAR-100-5x5}} & \multirow{3}{*}{Vanilla}        & Standard  & $54.04\%$   & $71.67\%$      & $75.64\%$  	\\
                         &                                 					& ADV       & $78.24\%$   & $64.92\%$      & $61.72\%$  	\\
                         &                                 					& TRADES    & $81.64\%$   & $68.96\%$      & $67.16\%$  	\\ \cline{2-6}
                         & \multirow{3}{*}{HR}   							& Standard  & $44.76\%$   & $82.52\%$      & $83.12\%$  	\\
                         &                                 					& ADV       & $87.80\%$   & $64.96\%$      & $73.44\%$  	\\
                         &                                 					& TRADES    & $84.36\%$   & $75.32\%$      & $65.88\%$  	\\\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}

\begin{table*}[h]
\begin{footnotesize}
\caption{Performance on CIFAR-10 and CIFAR100-subset against $\ell_{\infty}$ bounded transferred attacks ($\eps = 8/255$). }
\label{table:parent_attack}
%\vskip 0.15in
\begin{center}
\setlength{\tabcolsep}{15pt} % Default value: 6pt (space between columns)
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{tabular}{lllll}
                                    & Method	& Standard 	  & ADV 		   & TRADES 		\\ \Xhline{2\arrayrulewidth}
\multirow{3}{*}{CIFAR-10}    		& Standard  & $49.21\%$   & $92.63\%$      & $94.36\%$ 	 \\
                                    & ADV       & $95.36\%$   & $90.49\%$      & $93.14\%$  	 \\
                                    & TRADES    & $94.37\%$   & $90.89\%$      & $88.75\%$   	\\  \hline \hline

\multirow{3}{*}{CIFAR-100-5x5}      & Standard  & $44.76\%$   & $82.52\%$      & $83.12\%$  	\\
                                    & ADV       & $87.80\%$   & $64.96\%$      & $73.44\%$  	\\
                                    & TRADES    & $84.36\%$   & $75.32\%$      & $64.88\%$  	\\\Xhline{2\arrayrulewidth}
\end{tabular}
\end{center}
\end{footnotesize}
\end{table*}
